Volumetric Surfaces: Representing Fuzzy Geometries with Layered Meshes

High-quality view synthesis relies on volume rendering, splatting, or surface rendering. While surface rendering is typically the fastest, it struggles to accurately model fuzzy geometry like hair. In turn, alpha-blending techniques excel at representing fuzzy materials but require an unbounded number of samples per ray (P1). Further overheads are induced by empty space skipping in volume rendering (P2) and sorting input primitives in splatting (P3). We present a novel representation for real-time view synthesis where the (P1) number of sampling locations is small and bounded, (P2) sampling locations are efficiently found via rasterization, and (P3) rendering is sorting-free. We achieve this by representing objects as semi-transparent multi-layer meshes rendered in a fixed order. First, we model surface layers as signed distance function (SDF) shells with optimal spacing learned during training. Then, we bake them as meshes and fit UV textures. Unlike single-surface methods, our multi-layer representation effectively models fuzzy objects. In contrast to volume and splatting-based methods, our approach enables real-time rendering on low-power laptops and smartphones.

==> tables/datasets_tables.tex <==
\begin{table*}[h]
\centering
\caption{2DGS}
\label{tab:2dgs:base}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender & \cellcolor{tabthird} 34.613 & \cellcolor{tabsecond} 0.986 & \cellcolor{tabfirst} 0.038 &  31.782 & \cellcolor{tabsecond} 0.976 & \cellcolor{tabfirst} 0.046 \\ 
Custom &  34.401 &  0.974 &  0.184 & \cellcolor{tabthird} 32.788 &  0.965 &  0.190 \\ 
DTU & \cellcolor{tabfirst} 40.445 & \cellcolor{tabfirst} 0.994 & \cellcolor{tabsecond} 0.092 & \cellcolor{tabfirst} 38.459 & \cellcolor{tabfirst} 0.990 & \cellcolor{tabsecond} 0.101 \\ 
Shelly & \cellcolor{tabsecond} 36.565 & \cellcolor{tabthird} 0.983 & \cellcolor{tabthird} 0.104 & \cellcolor{tabsecond} 34.235 & \cellcolor{tabthird} 0.969 & \cellcolor{tabthird} 0.112 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3DGS}
\label{tab:3dgs:base}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender & \cellcolor{tabthird} 36.763 & \cellcolor{tabthird} 0.991 & \cellcolor{tabfirst} 0.030 &  33.227 & \cellcolor{tabthird} 0.981 & \cellcolor{tabfirst} 0.037 \\ 
Custom &  26.770 &  0.878 &  0.201 & \cellcolor{tabsecond} 37.345 & \cellcolor{tabsecond} 0.982 &  0.147 \\ 
DTU & \cellcolor{tabfirst} 42.338 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabsecond} 0.073 & \cellcolor{tabfirst} 38.060 & \cellcolor{tabfirst} 0.989 & \cellcolor{tabsecond} 0.086 \\ 
Shelly & \cellcolor{tabsecond} 38.853 & \cellcolor{tabsecond} 0.991 & \cellcolor{tabthird} 0.078 & \cellcolor{tabthird} 35.443 &  0.975 & \cellcolor{tabthird} 0.089 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{PermutoSDF}
\label{tab:permutosdf:base}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  29.311 & \cellcolor{tabsecond} 0.975 & \cellcolor{tabfirst} 0.057 &  28.052 & \cellcolor{tabsecond} 0.966 & \cellcolor{tabfirst} 0.065 \\ 
Custom & \cellcolor{tabsecond} 33.296 &  0.959 &  0.186 & \cellcolor{tabsecond} 32.940 &  0.945 &  0.192 \\ 
DTU & \cellcolor{tabfirst} 38.692 & \cellcolor{tabfirst} 0.992 & \cellcolor{tabsecond} 0.090 & \cellcolor{tabfirst} 36.312 & \cellcolor{tabfirst} 0.988 & \cellcolor{tabsecond} 0.098 \\ 
Shelly & \cellcolor{tabthird} 31.091 & \cellcolor{tabthird} 0.964 & \cellcolor{tabthird} 0.122 & \cellcolor{tabthird} 29.850 & \cellcolor{tabthird} 0.950 & \cellcolor{tabthird} 0.129 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{1-SDF}
\label{tab:offsets_surfs:base_1}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
Custom & \cellcolor{tabfirst} 34.362 & \cellcolor{tabfirst} 0.972 &  0.189 & \cellcolor{tabfirst} 33.486 & \cellcolor{tabfirst} 0.962 &  0.192 \\ 
DTU & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
Shelly & \cellcolor{tabsecond} 31.269 & \cellcolor{tabsecond} 0.961 & \cellcolor{tabthird} 0.130 & \cellcolor{tabsecond} 30.798 & \cellcolor{tabsecond} 0.953 & \cellcolor{tabthird} 0.134 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3-SDF}
\label{tab:offsets_surfs:base_3}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
Custom & \cellcolor{tabfirst} 36.006 & \cellcolor{tabfirst} 0.982 & \cellcolor{tabthird} 0.181 & \cellcolor{tabfirst} 35.087 & \cellcolor{tabfirst} 0.974 & \cellcolor{tabthird} 0.184 \\ 
DTU & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
Shelly & \cellcolor{tabsecond} 29.536 & \cellcolor{tabsecond} 0.933 &  0.209 & \cellcolor{tabsecond} 28.438 & \cellcolor{tabsecond} 0.909 &  0.227 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{5-SDF}
\label{tab:offsets_surfs:base_5}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
Custom & \cellcolor{tabfirst} 36.409 & \cellcolor{tabfirst} 0.983 &  0.167 & \cellcolor{tabfirst} 35.355 & \cellcolor{tabfirst} 0.971 &  0.176 \\ 
DTU & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
Shelly & \cellcolor{tabsecond} 32.498 & \cellcolor{tabsecond} 0.970 & \cellcolor{tabthird} 0.126 & \cellcolor{tabsecond} 32.046 & \cellcolor{tabsecond} 0.964 & \cellcolor{tabthird} 0.130 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{7-SDF}
\label{tab:offsets_surfs:base_7}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
Custom & \cellcolor{tabfirst} 36.756 & \cellcolor{tabfirst} 0.987 &  0.186 & \cellcolor{tabfirst} 35.964 & \cellcolor{tabfirst} 0.986 &  0.185 \\ 
DTU & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
Shelly & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabthird} 0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{9-SDF}
\label{tab:offsets_surfs:base_9}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
Custom & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
DTU & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabthird} 0.000 \\ 
Shelly & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{1-Mesh (baked)}
\label{tab:volsurfs:base_1_long}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
Custom & \cellcolor{tabfirst} 32.435 & \cellcolor{tabfirst} 0.960 &  0.181 & \cellcolor{tabfirst} 30.463 & \cellcolor{tabsecond} 0.933 &  0.188 \\ 
DTU & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
Shelly & \cellcolor{tabsecond} 28.879 & \cellcolor{tabsecond} 0.954 & \cellcolor{tabthird} 0.134 & \cellcolor{tabsecond} 28.533 & \cellcolor{tabfirst} 0.946 & \cellcolor{tabthird} 0.137 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3-Mesh (baked)}
\label{tab:volsurfs:base_3_long}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  32.255 & \cellcolor{tabthird} 0.982 & \cellcolor{tabfirst} 0.061 &  28.366 &  0.957 & \cellcolor{tabfirst} 0.085 \\ 
Custom & \cellcolor{tabsecond} 37.620 & \cellcolor{tabsecond} 0.989 &  0.160 & \cellcolor{tabsecond} 34.843 & \cellcolor{tabthird} 0.970 &  0.175 \\ 
DTU & \cellcolor{tabfirst} 40.784 & \cellcolor{tabfirst} 0.995 & \cellcolor{tabsecond} 0.077 & \cellcolor{tabfirst} 36.242 & \cellcolor{tabfirst} 0.984 & \cellcolor{tabsecond} 0.095 \\ 
Shelly & \cellcolor{tabthird} 33.799 &  0.982 & \cellcolor{tabthird} 0.112 & \cellcolor{tabthird} 32.873 & \cellcolor{tabsecond} 0.970 & \cellcolor{tabthird} 0.119 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{5-Mesh (baked)}
\label{tab:volsurfs:base_5_long}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  33.077 & \cellcolor{tabthird} 0.985 & \cellcolor{tabfirst} 0.056 &  28.644 &  0.958 & \cellcolor{tabfirst} 0.083 \\ 
Custom & \cellcolor{tabsecond} 38.141 & \cellcolor{tabsecond} 0.991 &  0.155 & \cellcolor{tabsecond} 35.419 & \cellcolor{tabthird} 0.974 &  0.171 \\ 
DTU & \cellcolor{tabfirst} 41.212 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabsecond} 0.072 & \cellcolor{tabfirst} 36.504 & \cellcolor{tabfirst} 0.985 & \cellcolor{tabsecond} 0.089 \\ 
Shelly & \cellcolor{tabthird} 34.592 &  0.984 & \cellcolor{tabthird} 0.110 & \cellcolor{tabthird} 34.098 & \cellcolor{tabsecond} 0.979 & \cellcolor{tabthird} 0.114 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{7-Mesh (baked)}
\label{tab:volsurfs:base_7_long}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  33.159 &  0.985 & \cellcolor{tabfirst} 0.057 &  28.748 &  0.959 & \cellcolor{tabfirst} 0.083 \\ 
Custom & \cellcolor{tabsecond} 38.222 & \cellcolor{tabsecond} 0.992 &  0.153 & \cellcolor{tabsecond} 35.605 & \cellcolor{tabthird} 0.976 &  0.169 \\ 
DTU & \cellcolor{tabfirst} 41.475 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabsecond} 0.071 & \cellcolor{tabfirst} 36.624 & \cellcolor{tabfirst} 0.987 & \cellcolor{tabsecond} 0.087 \\ 
Shelly & \cellcolor{tabthird} 34.816 & \cellcolor{tabthird} 0.985 & \cellcolor{tabthird} 0.109 & \cellcolor{tabthird} 34.331 & \cellcolor{tabsecond} 0.980 & \cellcolor{tabthird} 0.113 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{9-Mesh (baked)}
\label{tab:volsurfs:base_9_long}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
Blender &  33.044 &  0.985 & \cellcolor{tabfirst} 0.058 &  28.656 &  0.959 & \cellcolor{tabfirst} 0.084 \\ 
Custom & \cellcolor{tabsecond} 38.322 & \cellcolor{tabsecond} 0.992 &  0.151 & \cellcolor{tabsecond} 35.716 & \cellcolor{tabthird} 0.978 &  0.167 \\ 
DTU & \cellcolor{tabfirst} 41.745 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabsecond} 0.070 & \cellcolor{tabfirst} 36.826 & \cellcolor{tabfirst} 0.986 & \cellcolor{tabsecond} 0.086 \\ 
Shelly & \cellcolor{tabthird} 34.711 & \cellcolor{tabthird} 0.985 & \cellcolor{tabthird} 0.109 & \cellcolor{tabthird} 34.220 & \cellcolor{tabsecond} 0.981 & \cellcolor{tabthird} 0.113 \\ 
\bottomrule
\end{tabular}
\end{table*}



==> tables/methods_tables.tex <==
\begin{table*}[h]
\centering
\caption{DTU dataset}
\label{tab:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{method} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
3DGS & \cellcolor{tabfirst} 42.338 & \cellcolor{tabsecond} 0.996 &  0.073 & \cellcolor{tabsecond} 38.060 & \cellcolor{tabsecond} 0.989 &  0.086 \\ 
2DGS &  40.445 &  0.994 &  0.092 & \cellcolor{tabfirst} 38.459 & \cellcolor{tabfirst} 0.990 &  0.101 \\ 
PermutoSDF &  38.692 &  0.992 &  0.090 &  36.312 & \cellcolor{tabthird} 0.988 &  0.098 \\ 
1-SDF &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
3-SDF &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
5-SDF &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
7-SDF &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
9-SDF &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
1-Mesh (baked) &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
3-Mesh (baked) &  40.784 &  0.995 &  0.077 &  36.242 &  0.984 &  0.095 \\ 
5-Mesh (baked) &  41.212 &  0.996 &  0.072 &  36.504 &  0.985 &  0.089 \\ 
7-Mesh (baked) & \cellcolor{tabthird} 41.475 & \cellcolor{tabthird} 0.996 &  0.071 &  36.624 &  0.987 &  0.087 \\ 
9-Mesh (baked) & \cellcolor{tabsecond} 41.745 & \cellcolor{tabfirst} 0.996 &  0.070 & \cellcolor{tabthird} 36.826 &  0.986 &  0.086 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{Blender dataset}
\label{tab:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{method} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
3DGS & \cellcolor{tabfirst} 36.763 & \cellcolor{tabfirst} 0.991 &  0.030 & \cellcolor{tabfirst} 33.227 & \cellcolor{tabfirst} 0.981 &  0.037 \\ 
2DGS & \cellcolor{tabsecond} 34.613 & \cellcolor{tabsecond} 0.986 &  0.038 & \cellcolor{tabsecond} 31.782 & \cellcolor{tabsecond} 0.976 &  0.046 \\ 
PermutoSDF &  29.311 &  0.975 &  0.057 &  28.052 & \cellcolor{tabthird} 0.966 &  0.065 \\ 
1-SDF &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
3-SDF &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
5-SDF &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
7-SDF &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
9-SDF &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
1-Mesh (baked) &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
3-Mesh (baked) &  32.255 &  0.982 &  0.061 &  28.366 &  0.957 &  0.085 \\ 
5-Mesh (baked) &  33.077 &  0.985 &  0.056 &  28.644 &  0.958 &  0.083 \\ 
7-Mesh (baked) & \cellcolor{tabthird} 33.159 &  0.985 &  0.057 & \cellcolor{tabthird} 28.748 &  0.959 &  0.083 \\ 
9-Mesh (baked) &  33.044 & \cellcolor{tabthird} 0.985 &  0.058 &  28.656 &  0.959 &  0.084 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{Shelly dataset}
\label{tab:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{method} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
3DGS & \cellcolor{tabfirst} 38.853 & \cellcolor{tabfirst} 0.991 & \cellcolor{tabthird} 0.078 & \cellcolor{tabfirst} 35.443 &  0.975 & \cellcolor{tabthird} 0.089 \\ 
2DGS & \cellcolor{tabsecond} 36.565 &  0.983 &  0.104 & \cellcolor{tabthird} 34.235 &  0.969 &  0.112 \\ 
PermutoSDF &  31.091 &  0.964 &  0.122 &  29.850 &  0.950 &  0.129 \\ 
1-SDF &  31.269 &  0.961 &  0.130 &  30.798 &  0.953 &  0.134 \\ 
3-SDF &  29.536 &  0.933 &  0.209 &  28.438 &  0.909 &  0.227 \\ 
5-SDF &  32.498 &  0.970 &  0.126 &  32.046 &  0.964 &  0.130 \\ 
7-SDF &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
9-SDF &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
1-Mesh (baked) &  28.879 &  0.954 &  0.134 &  28.533 &  0.946 &  0.137 \\ 
3-Mesh (baked) &  33.799 &  0.982 &  0.112 &  32.873 &  0.970 &  0.119 \\ 
5-Mesh (baked) &  34.592 &  0.984 &  0.110 &  34.098 & \cellcolor{tabthird} 0.979 &  0.114 \\ 
7-Mesh (baked) & \cellcolor{tabthird} 34.816 & \cellcolor{tabthird} 0.985 &  0.109 & \cellcolor{tabsecond} 34.331 & \cellcolor{tabsecond} 0.980 &  0.113 \\ 
9-Mesh (baked) &  34.711 & \cellcolor{tabsecond} 0.985 &  0.109 &  34.220 & \cellcolor{tabfirst} 0.981 &  0.113 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{Custom dataset}
\label{tab:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{method} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
3DGS &  26.770 &  0.878 &  0.201 & \cellcolor{tabfirst} 37.345 & \cellcolor{tabsecond} 0.982 & \cellcolor{tabsecond} 0.147 \\ 
2DGS &  34.401 &  0.974 &  0.184 &  32.788 &  0.965 &  0.190 \\ 
PermutoSDF &  33.296 &  0.959 &  0.186 &  32.940 &  0.945 &  0.192 \\ 
1-SDF &  34.362 &  0.972 &  0.189 &  33.486 &  0.962 &  0.192 \\ 
3-SDF &  36.006 &  0.982 &  0.181 &  35.087 &  0.974 &  0.184 \\ 
5-SDF &  36.409 &  0.983 &  0.167 &  35.355 &  0.971 &  0.176 \\ 
7-SDF &  36.756 &  0.987 &  0.186 & \cellcolor{tabsecond} 35.964 & \cellcolor{tabfirst} 0.986 &  0.185 \\ 
9-SDF &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
1-Mesh (baked) &  32.435 &  0.960 &  0.181 &  30.463 &  0.933 &  0.188 \\ 
3-Mesh (baked) &  37.620 &  0.989 &  0.160 &  34.843 &  0.970 &  0.175 \\ 
5-Mesh (baked) & \cellcolor{tabthird} 38.141 & \cellcolor{tabthird} 0.991 &  0.155 &  35.419 &  0.974 &  0.171 \\ 
7-Mesh (baked) & \cellcolor{tabsecond} 38.222 & \cellcolor{tabsecond} 0.992 & \cellcolor{tabthird} 0.153 &  35.605 &  0.976 &  0.169 \\ 
9-Mesh (baked) & \cellcolor{tabfirst} 38.322 & \cellcolor{tabfirst} 0.992 & \cellcolor{tabsecond} 0.151 & \cellcolor{tabthird} 35.716 & \cellcolor{tabthird} 0.978 & \cellcolor{tabthird} 0.167 \\ 
\bottomrule
\end{tabular}
\end{table*}



==> tables/results_table_old.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{l|ccc|ccc|ccc}
        \toprule
        % & \multicolumn{3}{c|}{\textit{Shelly}~\cite{Wang2020SIGGRAPHASIA}} & \multicolumn{3}{c|}{\textit{NeRF-Synthetic}~\cite{Mildenhall2020ECCV}} & \multicolumn{3}{c}{\textit{Custom} (ours + \cite{Sharma2024ECCV})} \\
        & \multicolumn{3}{c|}{\textit{Shelly}~\cite{Wang2020SIGGRAPHASIA}} & \multicolumn{3}{c|}{\textit{Custom} (ours + \cite{Sharma2024ECCV})} & \multicolumn{3}{c}{\textit{NeRF-Synthetic}~\cite{Mildenhall2020ECCV}} \\
        \midrule
        \textit{method} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
        \midrule
        \cellcolor{tabrealtime}3DGS~\cite{Kerbl2023SIGGRAPH} & 
        \cellcolor{tabsecond} 35.443 & 0.964 & \cellcolor{tabfirst} 0.064 & 
        \cellcolor{tabfirst} 37.345  &  \cellcolor{tabfirst} 0.982 & \cellcolor{tabsecond} 0.147 &
        \cellcolor{tabfirst} 33.227 &  \cellcolor{tabfirst} 0.981 & \cellcolor{tabfirst} 0.037 \\
        % 2DGS & 
        % 34.235 &  0.969 & 0.112 & 
        % 31.782 &  0.976  & 0.046 & 
        % 32.788 &  0.965 & 0.189 \\ 
        Instant-NGP~\cite{Mueller2022SIGGRAPH} & 33.22 &  0.922 & 0.125 &
        31.133 &  0.935 & \cellcolor{tabfirst} 0.132 & 
        \cellcolor{tabsecond} 33.180 & / & / \\
        PermutoSDF~\cite{Rosu2023CVPR} & 
        29.850 & 0.950 &  0.129 &  
        33.306 &  0.961 & 0.193 &
        28.052 &  \cellcolor{tabsecond} 0.966 &  0.065 \\
        AdaptiveShells$^\star$~\cite{Wang2020SIGGRAPHASIA}  & 
        \cellcolor{tabfirst} 36.020 &  0.954 &  \cellcolor{tabthird} 0.079 & 
        / &  / & / &
        \cellcolor{tabthird} 31.840 &  0.957 &  \cellcolor{tabsecond} 0.056 \\
        QuadFields$^\star$~\cite{Sharma2024ECCV}  &  
        \cellcolor{tabthird} 35.130 &  0.954 &  \cellcolor{tabsecond} 0.073 & 
        / &  / & / &
        31.000 &  0.952 &  0.069 \\
        \cellcolor{tabrealtime}MobileNeRF~\cite{chen2023mobilenerf}  &  
        31.620 &  0.911 &  0.129 &    
        / &  / & / &
        30.900 &  0.947 &  \cellcolor{tabthird} 0.060 \\
        \midrule
        % 1-Mesh &  
        % 28.533 &  0.946 &  0.137 &  
        % / &  / &  / &  
        % / &  / & / \\
        3-Mesh &  
        33.247 &  0.977 &  0.118 &  
        34.843 &  0.970 &  0.175 &
        28.366 &  0.957 &  0.085 \\  
        5-Mesh &  
        34.098 &  \cellcolor{tabthird} 0.979 &  0.114 &  
        35.419 &  0.974 &  0.171 &  
        28.644 &  0.958 &  0.083 \\
        7-Mesh &  
        34.331 &  \cellcolor{tabsecond} 0.980 &  0.113 &  
        \cellcolor{tabthird} 35.605 &  \cellcolor{tabthird} 0.976 &  0.169 &  
        28.748 &  \cellcolor{tabthird} 0.959 &  0.083 \\ 
        9-Mesh &  
        34.220 &  \cellcolor{tabfirst} 0.981 &  0.113 &  
        \cellcolor{tabsecond} 35.716 & \cellcolor{tabsecond} 0.978 &  \cellcolor{tabthird} 0.167 &  %
        28.743 &  0.957 &  0.080 \\ % 
        \bottomrule
        \end{tabular}
    \caption{
    %
    \ste{Move NeRF-Synthetic results somewhere else? Remove them? Replace with DTU scenes 83, 105, plushy objects}
    %
    Results averaged across test scene.
    %
    Highlighted baselines meet the compute and/or memory requirements to run on general-purpose hardware (via WebGL) without modifications, as discussed in~\cref{sec:fast_rendering}.
    %
    Methods marked with a $\star$ show results from original papers, as code is unavailable. 
    %
    MobileNeRF and Instant-NGP results on Shelly from AdaptiveShells.
    %
    % Results marked with a $\circ$ use the Nerfstudio \cite{Tancik2023SIGGRAPH} implementation.
    %
    PermutoSDF trained until densities are fully peaked ($\phi_{\beta_3})$.
    %
    Metrics not provided by a baseline are denoted with “/”.
    %
    Please note that the Shelly dataset, as released by the authors, has a large overlap of views between test and training sets. All our experiments were conducted on a cleaned version of the dataset, free of this problem. However, a fair comparison with baselines whose code is not public remains difficult.
    %
    Our per-scene metrics are reported in the supplementary material.}
    % and results over the DTU datasets
    \label{tab:quantitative_image_1}
\end{table*}

==> tables/scenes_tables.tex <==
\begin{table*}[h]
\centering
\caption{2DGS, DTU dataset}
\label{tab:2dgs:base:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 38.837 & \cellcolor{tabsecond} 0.992 & \cellcolor{tabsecond} 0.110 & \cellcolor{tabsecond} 36.695 & \cellcolor{tabsecond} 0.987 & \cellcolor{tabsecond} 0.123 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 42.053 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabfirst} 0.074 & \cellcolor{tabfirst} 40.224 & \cellcolor{tabfirst} 0.993 & \cellcolor{tabfirst} 0.079 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{2DGS, Blender dataset}
\label{tab:2dgs:base:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair &  32.301 &  0.985 &  0.029 &  27.999 &  0.963 &  0.051 \\ 
drums &  28.795 &  0.976 &  0.041 &  26.025 &  0.963 &  0.048 \\ 
ficus & \cellcolor{tabsecond} 37.610 & \cellcolor{tabfirst} 0.997 & \cellcolor{tabsecond} 0.010 & \cellcolor{tabsecond} 35.181 & \cellcolor{tabsecond} 0.994 & \cellcolor{tabsecond} 0.014 \\ 
hotdog & \cellcolor{tabfirst} 39.330 & \cellcolor{tabthird} 0.996 &  0.027 & \cellcolor{tabfirst} 37.334 & \cellcolor{tabthird} 0.992 &  0.031 \\ 
lego &  35.588 &  0.995 & \cellcolor{tabthird} 0.021 &  32.548 &  0.989 & \cellcolor{tabthird} 0.029 \\ 
materials &  33.945 &  0.994 &  0.029 &  29.677 &  0.977 &  0.048 \\ 
mic & \cellcolor{tabthird} 36.860 & \cellcolor{tabsecond} 0.996 & \cellcolor{tabfirst} 0.006 & \cellcolor{tabthird} 34.661 & \cellcolor{tabfirst} 0.994 & \cellcolor{tabfirst} 0.009 \\ 
ship &  32.475 &  0.949 &  0.143 &  30.829 &  0.939 &  0.138 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{2DGS, Shelly dataset}
\label{tab:2dgs:base:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase & \cellcolor{tabthird} 38.105 & \cellcolor{tabsecond} 0.996 & \cellcolor{tabfirst} 0.040 &  34.073 & \cellcolor{tabthird} 0.985 & \cellcolor{tabsecond} 0.050 \\ 
horse & \cellcolor{tabfirst} 43.103 & \cellcolor{tabfirst} 0.999 & \cellcolor{tabsecond} 0.041 & \cellcolor{tabfirst} 39.996 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabfirst} 0.044 \\ 
khady &  31.346 &  0.944 &  0.200 &  29.377 &  0.905 &  0.228 \\ 
kitten & \cellcolor{tabsecond} 38.644 & \cellcolor{tabthird} 0.995 & \cellcolor{tabthird} 0.057 & \cellcolor{tabsecond} 36.819 & \cellcolor{tabsecond} 0.988 & \cellcolor{tabthird} 0.068 \\ 
pug &  35.900 &  0.982 &  0.133 & \cellcolor{tabthird} 34.226 &  0.974 &  0.125 \\ 
woolly &  32.289 &  0.980 &  0.151 &  30.918 &  0.967 &  0.158 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{2DGS, Custom dataset}
\label{tab:2dgs:base:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabfirst} 34.727 & \cellcolor{tabfirst} 0.983 & \cellcolor{tabfirst} 0.183 & \cellcolor{tabfirst} 34.375 & \cellcolor{tabfirst} 0.983 & \cellcolor{tabfirst} 0.181 \\ 
plushy & \cellcolor{tabsecond} 34.076 & \cellcolor{tabsecond} 0.966 & \cellcolor{tabsecond} 0.185 & \cellcolor{tabsecond} 31.201 & \cellcolor{tabsecond} 0.947 & \cellcolor{tabsecond} 0.198 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3DGS, DTU dataset}
\label{tab:3dgs:base:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 41.311 & \cellcolor{tabsecond} 0.996 & \cellcolor{tabsecond} 0.081 & \cellcolor{tabsecond} 35.505 & \cellcolor{tabsecond} 0.984 & \cellcolor{tabsecond} 0.102 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 43.366 & \cellcolor{tabfirst} 0.997 & \cellcolor{tabfirst} 0.064 & \cellcolor{tabfirst} 40.615 & \cellcolor{tabfirst} 0.994 & \cellcolor{tabfirst} 0.070 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3DGS, Blender dataset}
\label{tab:3dgs:base:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair &  38.957 &  0.998 & \cellcolor{tabthird} 0.010 & \cellcolor{tabthird} 35.464 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabthird} 0.015 \\ 
drums &  29.329 &  0.979 &  0.035 &  26.170 &  0.963 &  0.044 \\ 
ficus &  38.049 & \cellcolor{tabthird} 0.998 & \cellcolor{tabsecond} 0.007 &  34.904 & \cellcolor{tabthird} 0.994 & \cellcolor{tabsecond} 0.013 \\ 
hotdog & \cellcolor{tabfirst} 40.598 &  0.997 &  0.021 & \cellcolor{tabfirst} 37.577 &  0.992 &  0.026 \\ 
lego & \cellcolor{tabsecond} 39.734 & \cellcolor{tabsecond} 0.998 &  0.012 & \cellcolor{tabsecond} 35.789 &  0.993 &  0.019 \\ 
materials &  34.835 &  0.996 &  0.024 &  29.971 &  0.980 &  0.043 \\ 
mic & \cellcolor{tabthird} 39.089 & \cellcolor{tabfirst} 0.998 & \cellcolor{tabfirst} 0.005 &  35.063 & \cellcolor{tabsecond} 0.994 & \cellcolor{tabfirst} 0.009 \\ 
ship &  33.510 &  0.961 &  0.125 &  30.879 &  0.938 &  0.130 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3DGS, Shelly dataset}
\label{tab:3dgs:base:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase & \cellcolor{tabthird} 40.300 & \cellcolor{tabthird} 0.998 & \cellcolor{tabfirst} 0.029 &  34.821 & \cellcolor{tabthird} 0.986 & \cellcolor{tabsecond} 0.040 \\ 
horse & \cellcolor{tabfirst} 45.539 & \cellcolor{tabfirst} 0.999 & \cellcolor{tabsecond} 0.033 & \cellcolor{tabfirst} 41.451 & \cellcolor{tabfirst} 0.997 & \cellcolor{tabfirst} 0.038 \\ 
khady &  33.245 &  0.965 &  0.156 &  30.545 &  0.924 &  0.187 \\ 
kitten & \cellcolor{tabsecond} 40.942 & \cellcolor{tabsecond} 0.998 & \cellcolor{tabthird} 0.039 & \cellcolor{tabsecond} 38.169 & \cellcolor{tabsecond} 0.991 & \cellcolor{tabthird} 0.050 \\ 
pug &  38.820 &  0.994 &  0.092 & \cellcolor{tabthird} 35.959 &  0.983 &  0.089 \\ 
woolly &  34.271 &  0.991 &  0.117 &  31.710 &  0.969 &  0.130 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3DGS, Custom dataset}
\label{tab:3dgs:base:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabsecond} 14.597 & \cellcolor{tabsecond} 0.766 & \cellcolor{tabsecond} 0.260 & \cellcolor{tabfirst} 37.672 & \cellcolor{tabfirst} 0.990 & \cellcolor{tabfirst} 0.142 \\ 
plushy & \cellcolor{tabfirst} 38.942 & \cellcolor{tabfirst} 0.990 & \cellcolor{tabfirst} 0.141 & \cellcolor{tabsecond} 37.018 & \cellcolor{tabsecond} 0.975 & \cellcolor{tabsecond} 0.153 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{PermutoSDF, DTU dataset}
\label{tab:permutosdf:base:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 36.855 & \cellcolor{tabsecond} 0.990 & \cellcolor{tabsecond} 0.114 & \cellcolor{tabsecond} 34.783 & \cellcolor{tabsecond} 0.985 & \cellcolor{tabsecond} 0.124 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 40.530 & \cellcolor{tabfirst} 0.994 & \cellcolor{tabfirst} 0.067 & \cellcolor{tabfirst} 37.842 & \cellcolor{tabfirst} 0.991 & \cellcolor{tabfirst} 0.072 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{PermutoSDF, Blender dataset}
\label{tab:permutosdf:base:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair & \cellcolor{tabfirst} 33.604 & \cellcolor{tabfirst} 0.993 & \cellcolor{tabthird} 0.027 & \cellcolor{tabfirst} 32.437 & \cellcolor{tabfirst} 0.991 & \cellcolor{tabthird} 0.033 \\ 
drums &  24.581 &  0.944 &  0.096 &  23.220 &  0.937 &  0.100 \\ 
ficus &  29.238 & \cellcolor{tabthird} 0.984 &  0.046 &  28.160 & \cellcolor{tabthird} 0.977 &  0.054 \\ 
hotdog &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
lego & \cellcolor{tabthird} 29.414 &  0.975 &  0.064 & \cellcolor{tabthird} 28.527 &  0.969 &  0.071 \\ 
materials &  27.552 &  0.962 &  0.077 &  25.318 &  0.933 &  0.097 \\ 
mic & \cellcolor{tabsecond} 31.476 & \cellcolor{tabsecond} 0.989 &  0.030 & \cellcolor{tabsecond} 30.653 & \cellcolor{tabsecond} 0.987 &  0.033 \\ 
ship &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{PermutoSDF, Shelly dataset}
\label{tab:permutosdf:base:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase & \cellcolor{tabthird} 31.154 & \cellcolor{tabthird} 0.973 & \cellcolor{tabsecond} 0.068 &  28.424 &  0.953 & \cellcolor{tabsecond} 0.078 \\ 
horse & \cellcolor{tabfirst} 35.672 & \cellcolor{tabfirst} 0.995 & \cellcolor{tabfirst} 0.039 & \cellcolor{tabfirst} 34.677 & \cellcolor{tabfirst} 0.993 & \cellcolor{tabfirst} 0.040 \\ 
khady &  28.231 &  0.924 &  0.197 &  26.219 &  0.879 &  0.226 \\ 
kitten & \cellcolor{tabsecond} 31.653 & \cellcolor{tabsecond} 0.980 & \cellcolor{tabthird} 0.085 & \cellcolor{tabsecond} 30.913 & \cellcolor{tabsecond} 0.971 & \cellcolor{tabthird} 0.093 \\ 
pug &  30.156 &  0.961 &  0.175 & \cellcolor{tabthird} 29.480 & \cellcolor{tabthird} 0.953 &  0.168 \\ 
woolly &  29.678 &  0.952 &  0.169 &  29.387 &  0.949 &  0.167 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{PermutoSDF, Custom dataset}
\label{tab:permutosdf:base:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 \\ 
plushy & \cellcolor{tabfirst} 33.296 & \cellcolor{tabfirst} 0.959 & \cellcolor{tabsecond} 0.186 & \cellcolor{tabfirst} 32.940 & \cellcolor{tabfirst} 0.945 & \cellcolor{tabsecond} 0.192 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{1-SDF, DTU dataset}
\label{tab:offsets_surfs:base_1:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{1-SDF, Blender dataset}
\label{tab:offsets_surfs:base_1:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
drums &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
ficus &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
hotdog &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
lego &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
materials & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 \\ 
mic & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 \\ 
ship & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{1-SDF, Shelly dataset}
\label{tab:offsets_surfs:base_1:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase &  30.736 & \cellcolor{tabthird} 0.969 & \cellcolor{tabsecond} 0.072 &  29.936 &  0.963 & \cellcolor{tabsecond} 0.077 \\ 
horse & \cellcolor{tabfirst} 36.222 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabfirst} 0.041 & \cellcolor{tabfirst} 35.610 & \cellcolor{tabfirst} 0.995 & \cellcolor{tabfirst} 0.041 \\ 
khady &  28.504 &  0.925 &  0.207 &  27.415 &  0.897 &  0.227 \\ 
kitten & \cellcolor{tabsecond} 32.184 & \cellcolor{tabsecond} 0.981 & \cellcolor{tabthird} 0.085 & \cellcolor{tabsecond} 32.169 & \cellcolor{tabsecond} 0.979 & \cellcolor{tabthird} 0.091 \\ 
pug & \cellcolor{tabthird} 31.408 &  0.967 &  0.171 & \cellcolor{tabthird} 31.261 & \cellcolor{tabthird} 0.964 &  0.164 \\ 
woolly &  28.561 &  0.926 &  0.202 &  28.395 &  0.920 &  0.202 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{1-SDF, Custom dataset}
\label{tab:offsets_surfs:base_1:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabfirst} 34.390 & \cellcolor{tabfirst} 0.978 & \cellcolor{tabsecond} 0.195 & \cellcolor{tabfirst} 33.672 & \cellcolor{tabfirst} 0.977 & \cellcolor{tabsecond} 0.194 \\ 
plushy & \cellcolor{tabsecond} 34.334 & \cellcolor{tabsecond} 0.966 & \cellcolor{tabfirst} 0.183 & \cellcolor{tabsecond} 33.299 & \cellcolor{tabsecond} 0.946 & \cellcolor{tabfirst} 0.189 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3-SDF, DTU dataset}
\label{tab:offsets_surfs:base_3:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3-SDF, Blender dataset}
\label{tab:offsets_surfs:base_3:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
drums &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
ficus &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
hotdog &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
lego &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
materials & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 \\ 
mic & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 \\ 
ship & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3-SDF, Shelly dataset}
\label{tab:offsets_surfs:base_3:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
horse &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
khady & \cellcolor{tabfirst} 29.536 & \cellcolor{tabfirst} 0.933 &  0.209 & \cellcolor{tabfirst} 28.438 & \cellcolor{tabfirst} 0.909 &  0.227 \\ 
kitten &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
pug & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 \\ 
woolly & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3-SDF, Custom dataset}
\label{tab:offsets_surfs:base_3:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabfirst} 36.072 & \cellcolor{tabfirst} 0.984 & \cellcolor{tabsecond} 0.191 & \cellcolor{tabfirst} 35.342 & \cellcolor{tabfirst} 0.983 & \cellcolor{tabsecond} 0.190 \\ 
plushy & \cellcolor{tabsecond} 35.940 & \cellcolor{tabsecond} 0.980 & \cellcolor{tabfirst} 0.171 & \cellcolor{tabsecond} 34.832 & \cellcolor{tabsecond} 0.966 & \cellcolor{tabfirst} 0.179 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{5-SDF, DTU dataset}
\label{tab:offsets_surfs:base_5:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{5-SDF, Blender dataset}
\label{tab:offsets_surfs:base_5:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
drums &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
ficus &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
hotdog &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
lego &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
materials & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 \\ 
mic & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 \\ 
ship & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{5-SDF, Shelly dataset}
\label{tab:offsets_surfs:base_5:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase &  31.804 & \cellcolor{tabthird} 0.977 & \cellcolor{tabsecond} 0.071 &  31.076 &  0.972 & \cellcolor{tabsecond} 0.076 \\ 
horse & \cellcolor{tabfirst} 37.266 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabfirst} 0.041 & \cellcolor{tabfirst} 36.793 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabfirst} 0.040 \\ 
khady &  29.681 &  0.935 &  0.207 &  28.639 &  0.912 &  0.225 \\ 
kitten & \cellcolor{tabsecond} 34.320 & \cellcolor{tabsecond} 0.989 & \cellcolor{tabthird} 0.081 & \cellcolor{tabsecond} 34.270 & \cellcolor{tabsecond} 0.987 & \cellcolor{tabthird} 0.087 \\ 
pug & \cellcolor{tabthird} 32.643 &  0.975 &  0.166 & \cellcolor{tabthird} 32.344 & \cellcolor{tabthird} 0.972 &  0.160 \\ 
woolly &  29.271 &  0.947 &  0.193 &  29.154 &  0.946 &  0.191 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{5-SDF, Custom dataset}
\label{tab:offsets_surfs:base_5:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 \\ 
plushy & \cellcolor{tabfirst} 36.409 & \cellcolor{tabfirst} 0.983 & \cellcolor{tabsecond} 0.167 & \cellcolor{tabfirst} 35.355 & \cellcolor{tabfirst} 0.971 & \cellcolor{tabsecond} 0.176 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{7-SDF, DTU dataset}
\label{tab:offsets_surfs:base_7:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{7-SDF, Blender dataset}
\label{tab:offsets_surfs:base_7:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
drums &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
ficus &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
hotdog &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
lego &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
materials & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 \\ 
mic & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 \\ 
ship & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{7-SDF, Shelly dataset}
\label{tab:offsets_surfs:base_7:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
horse &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
khady &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
kitten & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 \\ 
pug & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 \\ 
woolly & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{7-SDF, Custom dataset}
\label{tab:offsets_surfs:base_7:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabfirst} 36.756 & \cellcolor{tabfirst} 0.987 & \cellcolor{tabsecond} 0.186 & \cellcolor{tabfirst} 35.964 & \cellcolor{tabfirst} 0.986 & \cellcolor{tabsecond} 0.185 \\ 
plushy & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{9-SDF, DTU dataset}
\label{tab:offsets_surfs:base_9:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{9-SDF, Blender dataset}
\label{tab:offsets_surfs:base_9:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
drums &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
ficus &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
hotdog &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
lego &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
materials & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 \\ 
mic & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 \\ 
ship & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{9-SDF, Shelly dataset}
\label{tab:offsets_surfs:base_9:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
horse &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
khady &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
kitten & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 \\ 
pug & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 \\ 
woolly & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{9-SDF, Custom dataset}
\label{tab:offsets_surfs:base_9:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 \\ 
plushy & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{1-Mesh (baked), DTU dataset}
\label{tab:volsurfs:base_1_long:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabsecond} 0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{1-Mesh (baked), Blender dataset}
\label{tab:volsurfs:base_1_long:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 &  0.000 &  0.000 & \cellcolor{tabfirst} 0.000 \\ 
drums &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 &  0.000 &  0.000 & \cellcolor{tabsecond} 0.000 \\ 
ficus &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 &  0.000 &  0.000 & \cellcolor{tabthird} 0.000 \\ 
hotdog &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
lego &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 &  0.000 \\ 
materials & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 & \cellcolor{tabthird} 0.000 & \cellcolor{tabthird} 0.000 &  0.000 \\ 
mic & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 & \cellcolor{tabsecond} 0.000 & \cellcolor{tabsecond} 0.000 &  0.000 \\ 
ship & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 & \cellcolor{tabfirst} 0.000 & \cellcolor{tabfirst} 0.000 &  0.000 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{1-Mesh (baked), Shelly dataset}
\label{tab:volsurfs:base_1_long:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase &  27.103 &  0.953 & \cellcolor{tabsecond} 0.082 &  26.542 &  0.947 & \cellcolor{tabsecond} 0.086 \\ 
horse &  28.791 & \cellcolor{tabsecond} 0.968 & \cellcolor{tabfirst} 0.071 &  28.597 & \cellcolor{tabfirst} 0.970 & \cellcolor{tabfirst} 0.066 \\ 
khady &  28.303 &  0.931 &  0.192 &  27.221 &  0.904 &  0.212 \\ 
kitten & \cellcolor{tabsecond} 29.361 & \cellcolor{tabthird} 0.953 & \cellcolor{tabthird} 0.091 & \cellcolor{tabsecond} 29.217 &  0.941 & \cellcolor{tabthird} 0.098 \\ 
pug & \cellcolor{tabfirst} 30.754 & \cellcolor{tabfirst} 0.970 &  0.163 & \cellcolor{tabfirst} 30.761 & \cellcolor{tabsecond} 0.968 &  0.155 \\ 
woolly & \cellcolor{tabthird} 28.959 &  0.948 &  0.204 & \cellcolor{tabthird} 28.862 & \cellcolor{tabthird} 0.947 &  0.203 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{1-Mesh (baked), Custom dataset}
\label{tab:volsurfs:base_1_long:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabsecond} 31.647 & \cellcolor{tabsecond} 0.956 & \cellcolor{tabsecond} 0.192 & \cellcolor{tabfirst} 30.895 & \cellcolor{tabfirst} 0.954 & \cellcolor{tabsecond} 0.191 \\ 
plushy & \cellcolor{tabfirst} 33.224 & \cellcolor{tabfirst} 0.964 & \cellcolor{tabfirst} 0.170 & \cellcolor{tabsecond} 30.031 & \cellcolor{tabsecond} 0.912 & \cellcolor{tabfirst} 0.185 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3-Mesh (baked), DTU dataset}
\label{tab:volsurfs:base_3_long:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 39.223 & \cellcolor{tabsecond} 0.994 & \cellcolor{tabsecond} 0.100 & \cellcolor{tabsecond} 34.607 & \cellcolor{tabsecond} 0.979 & \cellcolor{tabsecond} 0.123 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 42.346 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabfirst} 0.055 & \cellcolor{tabfirst} 37.878 & \cellcolor{tabfirst} 0.989 & \cellcolor{tabfirst} 0.066 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3-Mesh (baked), Blender dataset}
\label{tab:volsurfs:base_3_long:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair & \cellcolor{tabsecond} 35.354 & \cellcolor{tabfirst} 0.996 & \cellcolor{tabsecond} 0.027 & \cellcolor{tabthird} 31.602 & \cellcolor{tabfirst} 0.989 & \cellcolor{tabsecond} 0.043 \\ 
drums &  27.774 &  0.972 &  0.074 &  23.202 &  0.933 &  0.106 \\ 
ficus &  30.674 &  0.991 & \cellcolor{tabthird} 0.041 &  26.563 &  0.971 &  0.060 \\ 
hotdog & \cellcolor{tabfirst} 37.638 & \cellcolor{tabthird} 0.995 &  0.041 & \cellcolor{tabfirst} 34.874 & \cellcolor{tabthird} 0.984 & \cellcolor{tabthird} 0.057 \\ 
lego &  32.400 &  0.989 &  0.054 &  29.436 &  0.967 &  0.082 \\ 
materials &  30.985 &  0.990 &  0.058 &  24.839 &  0.940 &  0.096 \\ 
mic & \cellcolor{tabthird} 34.606 & \cellcolor{tabsecond} 0.995 & \cellcolor{tabfirst} 0.019 & \cellcolor{tabsecond} 31.798 & \cellcolor{tabsecond} 0.984 & \cellcolor{tabfirst} 0.036 \\ 
ship &  28.606 &  0.931 &  0.175 &  24.612 &  0.890 &  0.199 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3-Mesh (baked), Shelly dataset}
\label{tab:volsurfs:base_3_long:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase &  32.688 & \cellcolor{tabthird} 0.985 & \cellcolor{tabsecond} 0.064 &  32.261 & \cellcolor{tabthird} 0.984 & \cellcolor{tabsecond} 0.068 \\ 
horse & \cellcolor{tabfirst} 38.621 & \cellcolor{tabfirst} 0.997 & \cellcolor{tabfirst} 0.039 & \cellcolor{tabfirst} 38.175 & \cellcolor{tabfirst} 0.997 & \cellcolor{tabfirst} 0.039 \\ 
khady &  31.604 &  0.965 &  0.170 &  27.437 &  0.892 &  0.205 \\ 
kitten & \cellcolor{tabsecond} 35.761 & \cellcolor{tabsecond} 0.992 & \cellcolor{tabthird} 0.073 & \cellcolor{tabsecond} 35.681 & \cellcolor{tabsecond} 0.990 & \cellcolor{tabthird} 0.080 \\ 
pug & \cellcolor{tabthird} 33.872 &  0.983 &  0.148 & \cellcolor{tabthird} 33.569 &  0.982 &  0.141 \\ 
woolly &  30.248 &  0.971 &  0.179 &  30.118 &  0.972 &  0.179 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{3-Mesh (baked), Custom dataset}
\label{tab:volsurfs:base_3_long:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabsecond} 37.122 & \cellcolor{tabsecond} 0.987 & \cellcolor{tabsecond} 0.180 & \cellcolor{tabfirst} 35.433 & \cellcolor{tabfirst} 0.983 & \cellcolor{tabsecond} 0.182 \\ 
plushy & \cellcolor{tabfirst} 38.117 & \cellcolor{tabfirst} 0.991 & \cellcolor{tabfirst} 0.139 & \cellcolor{tabsecond} 34.252 & \cellcolor{tabsecond} 0.956 & \cellcolor{tabfirst} 0.168 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{5-Mesh (baked), DTU dataset}
\label{tab:volsurfs:base_5_long:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 39.682 & \cellcolor{tabsecond} 0.995 & \cellcolor{tabsecond} 0.092 & \cellcolor{tabsecond} 34.875 & \cellcolor{tabsecond} 0.980 & \cellcolor{tabsecond} 0.115 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 42.741 & \cellcolor{tabfirst} 0.997 & \cellcolor{tabfirst} 0.052 & \cellcolor{tabfirst} 38.132 & \cellcolor{tabfirst} 0.990 & \cellcolor{tabfirst} 0.063 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{5-Mesh (baked), Blender dataset}
\label{tab:volsurfs:base_5_long:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair & \cellcolor{tabsecond} 35.305 & \cellcolor{tabfirst} 0.997 & \cellcolor{tabsecond} 0.027 & \cellcolor{tabthird} 31.718 & \cellcolor{tabsecond} 0.987 & \cellcolor{tabsecond} 0.046 \\ 
drums &  28.307 &  0.976 &  0.071 &  23.402 &  0.934 &  0.107 \\ 
ficus &  34.129 &  0.995 & \cellcolor{tabthird} 0.030 &  27.215 &  0.971 &  0.058 \\ 
hotdog & \cellcolor{tabfirst} 37.592 & \cellcolor{tabthird} 0.996 &  0.034 & \cellcolor{tabfirst} 35.152 & \cellcolor{tabfirst} 0.987 & \cellcolor{tabthird} 0.048 \\ 
lego &  32.897 &  0.990 &  0.050 &  29.830 &  0.972 &  0.076 \\ 
materials &  32.592 &  0.993 &  0.050 &  25.252 &  0.941 &  0.093 \\ 
mic & \cellcolor{tabthird} 34.909 & \cellcolor{tabsecond} 0.996 & \cellcolor{tabfirst} 0.017 & \cellcolor{tabsecond} 31.808 & \cellcolor{tabthird} 0.984 & \cellcolor{tabfirst} 0.034 \\ 
ship &  28.883 &  0.935 &  0.171 &  24.772 &  0.888 &  0.198 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{5-Mesh (baked), Shelly dataset}
\label{tab:volsurfs:base_5_long:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase &  34.007 & \cellcolor{tabthird} 0.989 & \cellcolor{tabsecond} 0.062 &  33.518 & \cellcolor{tabthird} 0.987 & \cellcolor{tabsecond} 0.065 \\ 
horse & \cellcolor{tabfirst} 39.904 & \cellcolor{tabfirst} 0.998 & \cellcolor{tabfirst} 0.036 & \cellcolor{tabfirst} 39.668 & \cellcolor{tabfirst} 0.998 & \cellcolor{tabfirst} 0.035 \\ 
khady &  31.511 &  0.964 &  0.176 &  29.825 &  0.939 &  0.197 \\ 
kitten & \cellcolor{tabsecond} 36.861 & \cellcolor{tabsecond} 0.994 & \cellcolor{tabthird} 0.069 & \cellcolor{tabsecond} 36.739 & \cellcolor{tabsecond} 0.992 & \cellcolor{tabthird} 0.077 \\ 
pug & \cellcolor{tabthird} 34.299 &  0.986 &  0.145 & \cellcolor{tabthird} 34.014 &  0.985 &  0.138 \\ 
woolly &  30.971 &  0.976 &  0.171 &  30.825 &  0.976 &  0.172 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{5-Mesh (baked), Custom dataset}
\label{tab:volsurfs:base_5_long:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabsecond} 37.560 & \cellcolor{tabsecond} 0.989 & \cellcolor{tabsecond} 0.177 & \cellcolor{tabfirst} 35.894 & \cellcolor{tabfirst} 0.985 & \cellcolor{tabsecond} 0.180 \\ 
plushy & \cellcolor{tabfirst} 38.721 & \cellcolor{tabfirst} 0.993 & \cellcolor{tabfirst} 0.133 & \cellcolor{tabsecond} 34.944 & \cellcolor{tabsecond} 0.964 & \cellcolor{tabfirst} 0.163 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{7-Mesh (baked), DTU dataset}
\label{tab:volsurfs:base_7_long:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 39.868 & \cellcolor{tabsecond} 0.995 & \cellcolor{tabsecond} 0.091 & \cellcolor{tabsecond} 35.331 & \cellcolor{tabsecond} 0.983 & \cellcolor{tabsecond} 0.112 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 43.082 & \cellcolor{tabfirst} 0.997 & \cellcolor{tabfirst} 0.051 & \cellcolor{tabfirst} 37.918 & \cellcolor{tabfirst} 0.991 & \cellcolor{tabfirst} 0.062 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{7-Mesh (baked), Blender dataset}
\label{tab:volsurfs:base_7_long:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair & \cellcolor{tabsecond} 35.362 & \cellcolor{tabfirst} 0.997 & \cellcolor{tabsecond} 0.027 & \cellcolor{tabsecond} 32.407 & \cellcolor{tabfirst} 0.990 & \cellcolor{tabsecond} 0.043 \\ 
drums &  28.217 &  0.976 &  0.072 &  23.366 &  0.934 &  0.106 \\ 
ficus & \cellcolor{tabthird} 35.052 &  0.996 & \cellcolor{tabthird} 0.027 &  27.348 &  0.971 &  0.057 \\ 
hotdog & \cellcolor{tabfirst} 37.858 & \cellcolor{tabthird} 0.996 &  0.036 & \cellcolor{tabfirst} 35.377 & \cellcolor{tabsecond} 0.987 & \cellcolor{tabthird} 0.050 \\ 
lego &  32.239 &  0.989 &  0.053 &  29.392 &  0.971 &  0.079 \\ 
materials &  32.850 &  0.993 &  0.050 &  25.216 &  0.940 &  0.093 \\ 
mic &  34.952 & \cellcolor{tabsecond} 0.996 & \cellcolor{tabfirst} 0.016 & \cellcolor{tabthird} 31.766 & \cellcolor{tabthird} 0.984 & \cellcolor{tabfirst} 0.034 \\ 
ship &  28.741 &  0.934 &  0.174 &  25.110 &  0.894 &  0.199 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{7-Mesh (baked), Shelly dataset}
\label{tab:volsurfs:base_7_long:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase & \cellcolor{tabthird} 34.902 & \cellcolor{tabthird} 0.991 & \cellcolor{tabsecond} 0.060 & \cellcolor{tabthird} 34.420 & \cellcolor{tabthird} 0.990 & \cellcolor{tabsecond} 0.063 \\ 
horse & \cellcolor{tabfirst} 40.144 & \cellcolor{tabfirst} 0.998 & \cellcolor{tabfirst} 0.035 & \cellcolor{tabfirst} 39.896 & \cellcolor{tabfirst} 0.998 & \cellcolor{tabfirst} 0.034 \\ 
khady &  31.609 &  0.966 &  0.176 &  29.918 &  0.940 &  0.197 \\ 
kitten & \cellcolor{tabsecond} 37.047 & \cellcolor{tabsecond} 0.995 & \cellcolor{tabthird} 0.068 & \cellcolor{tabsecond} 37.022 & \cellcolor{tabsecond} 0.993 & \cellcolor{tabthird} 0.076 \\ 
pug &  34.256 &  0.985 &  0.146 &  33.984 &  0.984 &  0.139 \\ 
woolly &  30.935 &  0.976 &  0.167 &  30.746 &  0.977 &  0.167 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{7-Mesh (baked), Custom dataset}
\label{tab:volsurfs:base_7_long:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabsecond} 37.676 & \cellcolor{tabsecond} 0.990 & \cellcolor{tabsecond} 0.174 & \cellcolor{tabfirst} 36.081 & \cellcolor{tabfirst} 0.986 & \cellcolor{tabsecond} 0.177 \\ 
plushy & \cellcolor{tabfirst} 38.768 & \cellcolor{tabfirst} 0.994 & \cellcolor{tabfirst} 0.132 & \cellcolor{tabsecond} 35.129 & \cellcolor{tabsecond} 0.967 & \cellcolor{tabfirst} 0.162 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{9-Mesh (baked), DTU dataset}
\label{tab:volsurfs:base_9_long:dtu}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
dtu\_scan105* & \cellcolor{tabsecond} 40.033 & \cellcolor{tabsecond} 0.995 & \cellcolor{tabsecond} 0.089 & \cellcolor{tabsecond} 35.191 & \cellcolor{tabsecond} 0.982 & \cellcolor{tabsecond} 0.111 \\ 
dtu\_scan83* & \cellcolor{tabfirst} 43.458 & \cellcolor{tabfirst} 0.998 & \cellcolor{tabfirst} 0.050 & \cellcolor{tabfirst} 38.461 & \cellcolor{tabfirst} 0.990 & \cellcolor{tabfirst} 0.062 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{9-Mesh (baked), Blender dataset}
\label{tab:volsurfs:base_9_long:blender}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
chair & \cellcolor{tabsecond} 35.496 & \cellcolor{tabfirst} 0.997 & \cellcolor{tabsecond} 0.026 & \cellcolor{tabsecond} 32.723 & \cellcolor{tabfirst} 0.990 & \cellcolor{tabsecond} 0.041 \\ 
drums &  28.193 &  0.976 &  0.075 &  23.205 &  0.933 &  0.111 \\ 
ficus & \cellcolor{tabthird} 35.119 &  0.996 & \cellcolor{tabthird} 0.027 &  27.341 &  0.971 &  0.058 \\ 
hotdog & \cellcolor{tabfirst} 37.498 & \cellcolor{tabthird} 0.996 &  0.037 & \cellcolor{tabfirst} 35.006 & \cellcolor{tabsecond} 0.987 & \cellcolor{tabthird} 0.053 \\ 
lego &  33.159 &  0.990 &  0.050 &  29.925 &  0.973 &  0.076 \\ 
materials &  31.554 &  0.991 &  0.053 &  25.335 &  0.944 &  0.091 \\ 
mic &  34.531 & \cellcolor{tabsecond} 0.996 & \cellcolor{tabfirst} 0.018 & \cellcolor{tabthird} 31.016 & \cellcolor{tabthird} 0.981 & \cellcolor{tabfirst} 0.039 \\ 
ship &  28.801 &  0.936 &  0.175 &  24.700 &  0.889 &  0.203 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{9-Mesh (baked), Shelly dataset}
\label{tab:volsurfs:base_9_long:shelly}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
fernvase & \cellcolor{tabthird} 34.976 & \cellcolor{tabthird} 0.992 & \cellcolor{tabsecond} 0.059 & \cellcolor{tabthird} 34.531 & \cellcolor{tabthird} 0.991 & \cellcolor{tabsecond} 0.063 \\ 
horse & \cellcolor{tabfirst} 39.418 & \cellcolor{tabfirst} 0.998 & \cellcolor{tabfirst} 0.035 & \cellcolor{tabfirst} 39.120 & \cellcolor{tabfirst} 0.998 & \cellcolor{tabfirst} 0.035 \\ 
khady &  31.546 &  0.966 &  0.177 &  29.927 &  0.942 &  0.198 \\ 
kitten & \cellcolor{tabsecond} 37.035 & \cellcolor{tabsecond} 0.995 & \cellcolor{tabthird} 0.068 & \cellcolor{tabsecond} 36.946 & \cellcolor{tabsecond} 0.993 & \cellcolor{tabthird} 0.076 \\ 
pug &  34.313 &  0.985 &  0.146 &  33.994 &  0.984 &  0.140 \\ 
woolly &  30.977 &  0.976 &  0.167 &  30.799 &  0.976 &  0.167 \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[h]
\centering
\caption{9-Mesh (baked), Custom dataset}
\label{tab:volsurfs:base_9_long:blendernerf}
\begin{tabular}{l|ccc|ccc}
\toprule
& & \textit{train} & & & \textit{test} & \\ 
\midrule
\textit{scene} & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
\midrule
hairy\_monkey & \cellcolor{tabsecond} 37.757 & \cellcolor{tabsecond} 0.991 & \cellcolor{tabsecond} 0.171 & \cellcolor{tabfirst} 36.130 & \cellcolor{tabfirst} 0.987 & \cellcolor{tabsecond} 0.175 \\ 
plushy & \cellcolor{tabfirst} 38.887 & \cellcolor{tabfirst} 0.994 & \cellcolor{tabfirst} 0.130 & \cellcolor{tabsecond} 35.301 & \cellcolor{tabsecond} 0.969 & \cellcolor{tabfirst} 0.160 \\ 
\bottomrule
\end{tabular}
\end{table*}



==> tables/textures_res_old.tex <==
\begin{table*}[t]
\begin{tabular}{l|ccccc|ccccc|ccccc}
\toprule
\multicolumn{16}{c}{\textit{train}} \\
\midrule
& \multicolumn{5}{c|}{PSNR $\uparrow$} & \multicolumn{5}{c|}{SSIM $\uparrow$} & \multicolumn{5}{c}{LPIPS $\downarrow$} \\
\midrule
\textit{k} & 
\multicolumn{1}{c}{mixed} & \multicolumn{1}{c}{2048} & \multicolumn{1}{c}{1024} & \multicolumn{1}{c}{512} & \multicolumn{1}{c|}{256} & 
\multicolumn{1}{c}{mixed} & \multicolumn{1}{c}{2048} & \multicolumn{1}{c}{1024} & \multicolumn{1}{c}{512} & \multicolumn{1}{c|}{256} & 
\multicolumn{1}{c}{mixed} & \multicolumn{1}{c}{2048} & \multicolumn{1}{c}{1024} & \multicolumn{1}{c}{512} & \multicolumn{1}{c}{256} \\
\midrule
% 1 & 
% / & / & / & / & / & % PSNR
% / & / & / & / & / & % SSIM
% / & / & / & / & / \\ % LPIPS   
3 & 
31.26 & 31.21 & 31.30 & 30.19 & 30.82 & % PSNR
0.96 & 0.96 & 0.96 &  0.96 & 0.95 & % SSIM
0.18 & 0.17 & 0.17 & 0.19 & 0.21 \\ % LPIPS  
5 & 
31.51 & 31.47 & 31.54 & 31.44 & 31.06 & % PSNR
0.96 & 0.96 & 0.96 &  0.96 & 0.95 & % SSIM
0.18 & 0.17 & 0.17 &  0.18 & 0.20 \\ % LPIPS  
7 & 
\cellcolor{tabfirst} 31.61 & 31.57 & 31.64 & 31.54 & 31.16  & % PSNR
0.97 & 0.96 & 0.96 & 0.96 & 0.96 & % SSIM
0.17 & 0.17 & 0.17 & 0.18 & 0.20 \\ % LPIPS  
9 & 
31.54 & 31.50 & 31.58 & 31.48 & 31.13 & % PSNR
0.97 & 0.97 & 0.97 & 0.96 & 0.96 & % SSIM
0.18 & 0.17 & 0.173 & 0.18 & 0.20 \\ % LPIPS  
\bottomrule
\end{tabular}

\vspace*{5mm}

\begin{tabular}{l|ccccc|ccccc|ccccc}
\toprule
\multicolumn{16}{c}{\textit{test}} \\
\midrule
& \multicolumn{5}{c|}{PSNR $\uparrow$} & \multicolumn{5}{c|}{SSIM $\uparrow$} & \multicolumn{5}{c}{LPIPS $\downarrow$} \\
\midrule
\textit{k} & 
\multicolumn{1}{c}{mixed} & \multicolumn{1}{c}{2048} & \multicolumn{1}{c}{1024} & \multicolumn{1}{c}{512} & \multicolumn{1}{c|}{256} & 
\multicolumn{1}{c}{mixed} & \multicolumn{1}{c}{2048} & \multicolumn{1}{c}{1024} & \multicolumn{1}{c}{512} & \multicolumn{1}{c|}{256} & 
\multicolumn{1}{c}{mixed} & \multicolumn{1}{c}{2048} & \multicolumn{1}{c}{1024} & \multicolumn{1}{c}{512} & \multicolumn{1}{c}{256} \\
\midrule
% 1 & 
% / & / & / & / & / & % PSNR
% / & / & / & / & / & % SSIM
% / & / & / & / & / \\ % LPIPS   
3 & 
29.64 & 29.63 & 29.67 & 29.59 & 29.30 & % PSNR
0.94 & 0.94 & 0.94 & 0.94 & 0.92 & % SSIM
0.20 & 0.19 & 0.19 & 0.20 & 0.22 \\ % LPIPS  
5 & 
29.82 & 29.82 & 29.85 & 29.76 & 29.48 & % PSNR
0.94 & 0.94 & 0.94 &  0.94 & 0.93 & % SSIM
0.20 & 0.19 & 0.20 &  0.20 & 0.22 \\ % LPIPS  
7 & 
29.91 & 29.91 & 29.95 & 29.87 & 29.58 & % PSNR
0.94 & 0.94 & 0.93 & 0.94 & 0.93 & % SSIM
0.20 & 0.19 & 0.19 & 0.20 & 0.22 \\ % LPIPS  
9 & 
29.93 & 29.90 & \cellcolor{tabfirst} 29.94 & 28.87 & 29.59 & % PSNR
0.94 & 0.94 & 0.94 & 0.94 & 0.93 & % SSIM
0.20 &  0.19 & 0.19 & 0.20 & 0.22 \\ % LPIPS  
\bottomrule
\end{tabular}

\caption{Results are on the \emph{Khady} scene from Shelly~\cite{Wang2020SIGGRAPHASIA}. Quantitative metrics when sweeping over the number of surfaces $k$ and target textures resolutions. Mixed resolutions are described in Sec. \ref{sec:meshes_texturing}. \ste{Note how increasing the number of surfaces improves the overall representation capacity on training views and generalization on test views.}}
\label{tab:textures_res}
\end{table*}
